A Mathematical Framework for Evaluation of SOAR Tools with Limited Survey Data

Security operation centers (SOCs) all over the world are tasked with reacting to cybersecurity alerts ranging in severity. Security Orchestration, Automation, and Response (SOAR) tools streamline cybersecurity alert responses by SOC operators. SOAR tool adoption is expensive both in effort and finances. Hence, it is crucial to limit adoption to those most worthwhile; yet no research evaluating or comparing SOAR tools exists. The goal of this work is to evaluate several SOAR tools using specific criteria pertaining to their usability. SOC operators were asked to first complete a survey about what SOAR tool aspects are most important. Operators were then assigned a set of SOAR tools for which they viewed demonstration and overview videos, and then operators completed a second survey wherein they were tasked with evaluating each of the tools on the aspects from the first survey. In addition, operators provided an overall rating to each of their assigned tools, and provided a ranking of their tools in order of preference. Due to time constraints on SOC operators for thorough testing, we provide a systematic method of downselecting a large pool of SOAR tools to a select few that merit next-step hands-on evaluation by SOC operators. Furthermore, the analyses conducted in this survey help to inform future development of SOAR tools to ensure that the appropriate functions are available for use in a SOC.

==> 10-intro.tex <==
\section{Introduction and Background}
\label{sec:intro} 
The term \textit{security operations center} (SOC) refers to the subteam of an organization's IT department tasked with maintaining the network's cyber health---the confidentiality, integrity, and availability of the enterprise's data and systems.
SOCs are now equipped with a widespread collection of data from a vast array of sensors feeding logs, alerts, and raw data to a security information and event management system (SIEM). SIEMs and back-end infrastructure generally provide SOCs customizable, real-time dashboards and rapid data query. However, the process of identifying incidents, responding appropriately, and documenting findings remains to be done by the operators. This leaves them with a tedious, manual effort often comprised of ill-defined workflows, navigating disparate systems and a sea of data, and is proving vastly inefficient. %Because SOAR tools must interact with each SOC's unique data feeds and systems and be configured to systematize and automate SOC-specific procedures, the adoption of a SOAR tool is costly in the training of operators, monetary cost, and technological debt.
\todo{The Introduction section should present to the reader the organization of the rest of the paper}
\todo{Does similar previous work exist in the bibliography? Is the cybersecurity industry currently adopting evaluation methodologies and/or related user acceptance assessment procedures?. If this is the case, it would be important to emphasise the proposal's strengths against these. }
\todo{It would also be interesting to know whether previous studies perceive similar patterns of acceptance from the end-user perspective.}
\todo{It is possible to estimate some kind of decision bias in the review board? Note that close organizations and experts tend to share a similar vision on their operational needs). }
\todo{The study focuses on user acceptance. It would be interesting to combine such a view with objective technical parameters, such as performance tests, efficiency, fault tolerance, resilience, etc. This could go from reinforcing the quality of the assessment of the solutions analysed, to highlighting points for improvement in the study process (for example, to what extent has the user been "convinced" by the video demonstration of the virtues of each solution, or which operational aspects are most valued with respect to the technical capabilities that enable them?}
\todo{its strengths and weaknesses are barely discussed in relation to previous work, which gives rise to the following suggestions.}
\todo{The specific contributions of this research should be better reflected in the introductory section.}
\todo{ It is not completely clear the rationale behind the selection of demographic attributes and the impact they had in the overall assessment. At a glance, and based on the questionnaire presented, only three were considered (Questions 1 to 3). Question 4 is rather an instruction by the way.}
\todo{ Although the authors claim no similar SOAR assessment methodology is found in the literature, authors are encouraged to cite evaluation approaches outside thorough cyber tools testing, such as those grounded in sentiment analysis or in operator's quality expectations.}
\todo{the main downside of this research is the lack of a common baseline to profile the quality requirements for the videos provided by the SOAR vendors. Authors are encouraged to extend more on this.}
Thus Security orchestration, automation, and response (SOAR) tools are a transformational and centerpiece tool for a SOC promising measurable gains in effectiveness and efficiency. This work will provide an in-progress report on the first-ever user study to assess and compare user preferences of SOAR tools with the aim of down selecting to a smaller number of tools to be extensively tested. % usability and SOC user preferences of SOAR tools. Our goal is to provide scientific assistance to an organization to winnow the wide variety of SOAR tools to the best one for the organization's needs. 

\subsubsection{SOAR Tools.}
SOAR tools are the newest generation of software tools designed to enable SOC operators to more efficiently and uniformly detect and address cybersecurity threats. 
We determined that for our purposes, a SOAR tool must have the following defining capabilities: 
(1) ingests a wide variety of SOC data, 
(2) assists in prioritizing, organizing, and displaying the data to the users, 
(3) allows customizable workflows or ``playbooks'' to standardize SOC procedures, 
(4) provides automation to expedite the SOC's procedures, 
(5) integrates with a ticketing system, and 
(6) facilitates collaboration of operators, potentially in disparate geographic locations or networks. 
%\citep{gartner_inc}. 
The capabilities of a SOAR tool are observed with the integration of a SOAR mechanism to secure energy microgrids--- wherein the tool collects and contextualizes security data from multiple sources in the microgrid, performs an overall sweep of the system to identify present vulnerabilities, and initialize or engage a response to detected threats \citep{microgrid}.

In some cases, the gap between SIEM environments and SOAR tools is more a matter of automation. For example, an AI-based SIEM that uses deep learning to dwindle the vast pool of would-be alerts into a more manageable set of alerts most likely to be true positives has been proposed \citep{AI_SOAR}. The ``threat intelligence'' capacity stores context about each incoming threat and whether it was deemed to be true/false positive in a repository that can be queried. If the threat is determined to be true, responses are executed automatically via playbook instructions \citep{AI_SOAR}.
%In Vast et al. (2021), the authors propose an AI-based SIEM that uses deep learning to dwindle the vast pool of would-be alerts into a more manageable set of alerts most likely to be true positives. 

Because SOAR tools are so new, with the term only being coined by Gartner in 2017 \citep{BREWER20198}, there is little research assessing their usability or the degree to which they improve SOC operators' ability to respond to threats. These tools are a joint application of both security orchestration and automation. Even though these two processes are often marketed together, they do have distinct functions that are worthy of note \citep{islam_babar_nepal_2019}. In general, the two can be distinguished as follows: \textit{orchestration} specifically refers to the integration of separate tools with different functions into a single platform to streamline and accelerate the investigation of a threat; \textit{automation} refers to reducing the manual effort required by SOC operators during investigation and threat response phase \citep{Microsoft}. Typically, automation will follow as a result of orchestration \citep{islam_babar_nepal_2019}.

\subsubsection{SOC workflow.}
%\todo{change this name}
We look for SOAR tools to help improve SOC efficiency by mitigating some of the costs of a false positive. The false positive rates that SOC analysts have to manage in a typical SIEM environment are extraordinarily high and impose a heavy burden on operators to identify which are credible threats. SIEM systems, along with other tools' operators have to monitor like intrusion detection systems and firewalls, do not provide a complete view of the entire security landscape, leading to extended threat detection and response times and reduced ability to prevent or quickly mitigate an attack \citep{Network, islam_babar_nepal_2019}. SOAR tools aim to help with this by speeding up and automating parts of an investigation, and helping SOC operators prioritize alerts to investigate.

Furthermore, SOC efficiency suffers due to time spent by the operators documenting findings in a readable fashion, collecting evidence across an array of sources, and completing other administrative-type procedures \citep{BREWER20198}. It is no surprise that improving efficiency largely goes hand-in-hand with subsidizing human operator duties with machine-based tasks.
% Because SOAR tools are marketed as doing so many distinct things, direct comparison of these commercially available tools is highly nontrivial. Such a study requires SOC operators to use them in a hands-on fashion. This is a complicated scientific effort that requires the establishment of a high-fidelity testing environment with metrics to gauge gains in efficiency and effectiveness. Additionally, sufficient time must be allocated to the SOC operators for both familiarization with the tool and the completion of a rigorous evaluation of the tools.

\subsubsection{Our contributions.}
Given all this, a first step for evaluating SOAR tools---and the focus of this work---is down-sampling the variety of tools to a subset worthy of the costly hands-on evaluation without discarding a potentially desired tool. 
% The focus of this work is to describe our mathematically-driven approach to equipping the sponsor organization with data needed to eliminating SOAR tools for hands-on evaluation.
We describe both our experimental design methodology and anonymized results---as a prerequisite, SOAR vendors agreed to providing licenses and support for this study in exchange for anonymity of their results and participation---of actual SOC operators evaluating 11 market-leading SOAR tools based on vendor-supplied technological overviews. 
% This describes the ``first half" of a larger, in-progress study that will culminate in the aforementioned hands-on tests of the fewer selected tools. 
% Our approach addresses each design concern mathematically with a goal of equipping the sponsor organization to make data-driven decisions with multiple views of the data. 
% Our contributions can be dichotomized into specific findings relevant to SOAR tools and reusable, novel data-analytic approaches to design questions and results analysis. 

In terms of understanding usability of SOAR tools, this work aids in understanding what defining capabilities are most desired by SOC operators and how this affects their preferences. 
Our unique pipeline provides a method for narrowing thorough testing down to only the tools that are most preferred by SOC operators. 
This pipeline's many unique and modular components could be applicable to future user studies, in particular: 
statistical simulations to quantify confidence of results under varying number of participants;
a novel algorithm for optimizing participant assignments; 
a framework for optimizing combinations and variants of multi-criteria recommender system (for predicting missing ratings) to the data at hand that outperforms the previous versions; 
an evaluation of supervised regressors for predicting overall ratings from aspect ratings is provided (and verifies that this is a needed step as it greatly out-performs predictions from the recommender system); 
many methods for ranking the tools based on the data are provided side-by-side including a novel application of PageRank to convert ratings data to ranking data; 
statistical analyses that investigate correlations present. 
To assist the community in reusing any of these methods, code will be released \href{https://github.com/noremsa/SurveyAnalysisFramework}{here} once open-source copyright is gained. 

In summation, this work will present a novel pipeline of ingesting sparse data and using a mathematically sound method to fully populate the matrix of data. Novel methods are then applied to create multiple views of data along with the statistical relevance of demographic factors. This paper will fill a gap in knowledge where we start with a survey of what the users of these tools actually want, and will proceed to an in depth user study of what the tools deliver.
%Thus, this work fills a gap where we start with a survey of what the users of these tools actually want, and will proceed to an in depth user study of what the tools deliver.
% In our experimental design, we address questions of how many operators, how to assign SOAR tool reviews to operators, how to address missing ratings, and how to leverage all received data in order to rank the 11 tools for next-step testing.
% However, because of constraints on operator availability, we assigned each operator only a subset for evaluation. As such, not every operator will complete the survey for every tool. 
% Thus, to confidently downselect the tools, we utilize multicriteria recommender systems to predict how users would rate aspects of tools they did not review, based on how similarly they reviewed tools that other operators provided feedback for. Next, we used machine learning to predict each SOC operators overall rating of each tool. Finally, we used Page Rank algorithm to find an overall ranking of the tools.
% More specifically, while realistic test environments were implemented for a hands-on study, 
% we established a systematic method to downselect from a wide range of SOAR tools to the most preferred few was developed to ensure resources in future testing focus on the tools which best met the SOC operators' needs.
% Job responsibilities of operators are dependent on SOC and the tier of the operator. As a tier 1 analyst, tasks might include reviewing blacklisted IP communications and daily reports, responding and triaging alerts from security information and event management (SIEM) tools, and responding to phishing emails. A tier 2 analyst might be tasked with analyzing emerging threat reports, developing security dashboards, and responding to incidents. Some of the metrics used for SOC analysts could include remediation of vulnerabilities, emails investigated, perimeters defended, and intrusion detection systems monitored. While some of these tasks seem intrinsically human, some of them are ripe for automation with a SOAR tool. 
%SOAR tools function similar to incident tracking tools and enable cybersecurity threats to be efficient, without sacrificing the quality, of responses. For our experiment, we requested that SOAR tools submitting have the following capabilities:
% \begin{enumerate}
% \item ingest a wide variety of logs/alerts
% \item rank and display logs/alerts. This may involve correlating/grouping events.
% \item provide playbooks/workflows (decision trees that guide analyst through the correct set of steps)
% \item automate repetitive tasks, such as steps of a playbook or ticketing actions
% \item integrate with a ticketing system and fill out/append data to tickets
% \item facilitate collaboration across SOC operators, possibly across networks, and both synchronously and asynchronously
% \end{enumerate}
% Based on this information, we determined specific aspects on which operators could evaluate these SOAR tools. 
% Prior to SOAR tool evaluation, we tasked the operators to rank which of these aspects are most important to them, with the anticipation that they would favor tools that performed well on these aspects. 

==> 20-related-work.tex <==
%\section{Related Works}
% \add{Since  our work is a user study of SOC operators on SOAR tools, i recommend changing this related works to only users studies on SOCs and anything regarding a SOAR tool. I don't believe any such work has been done! so i think we can quickly move on. I suggest saying "there are many previous user studies on SOC personnel, the difficulties with their job, and their tools [cite blah blah]. in fact there are only a few works that even mention SOAR tools [cite blah blah] \\ I like the SOAR tool descriptions and motivation paragraphs with references, but they are a bit wordy as is. Recommend we keep them but condensify and work it in the intro where i defined the SOAR tool via the 6 characteristics. 
%Here we explore previous works that served to provide relevant background on SOAR tool development, as well as to inform our methods for handling missing data.
%\todo{while i agree this is what our work does, i think we don't make this gap apparent until this sentence}
% \subsection{Recommender Systems}
% Since operators recruited for this survey were assigned a subset of the tools to review, this means that we have missing data since every operator did not complete the survey for each tool. This section provides a linear progression of previous research that informs our approach followed by our algorithm for filling in missing values to populate a complete dataset. 
% Consider a vector, $\vec{r}(u, t)$, that comprises the ratings assigned by user $u$ to tool $t$. Breese et al. \cite{breese1998empirical} considers the single-criteria problem where $\vec{r}(u,t)$ is a single number. Unknown values are defined as follows, 
% \begin{equation}
%     \label{eq:breese}
%     \vec{r}(u,t): = \frac{1}{\sum_{v\in \text{Users}} \s(u,v) } \sum_{v\in \text{Users}} \s(u,v) r(v,t)
% \end{equation}
% where $\s(u,v)$ is a similarity measure of users $u$ and $v$ computed with a standard similarity measure (e.g, cosine, inverse Euclidean, Pearson correlation) applied to the vector of ratings from $u$ and $v$ on the set of items both users rated. 
% % This can be conceptualized as an expectation where likelihood is proportional user similarity. 
% % More generally, the fundamental concept put forward (that we leverage heavily) is called collaborative filtering---that a user's ratings are predicted based on (in this case proportional to) ratings of those of other users with similar ratings. 
% Adomavicius \& Kwon (AK) \cite{adomavicius2007new} extend this framework to multi-criteria ratings where $\vec{r}(u,t)$ is a vector with $\vec{r}(u,t,n)$ user $u$'s overall rating of tool $t$ on the $n^{th}$ aspect. 
% Setting a distance on rating vectors, $d_R(\vec{r}(u,t), \vec{r}(v,s))$, %($\ell^p$ and Mahalanobis distance are tested), 
% AK defines the distance between two users, $u, v$, as 
% \begin{equation}
%     \label{eq:distance}
%     d_{U}(u,v) = \sum_{t\in T_{u,v}} d_R(\vec{r}(u,t), \vec{r}(v,t)) /|T_{u,v}|
% \end{equation}
% where $T_{u,v}:= \{$tools $t$ rated by both $u$ and $v$\}. 

% The similarity of two users is simply an inverse function of their distance such that $\s(u,v):= 1/(1+d_{U}(u,v))$.  
% Notably, the general framework is symmetric in users and items; hence, item similarity could just as easily produce predicted missing values. 
% Finally, for each missing aspect rating ($j = 1, ..., n-1$) $\vec{r}(u,t,j)$ is predicted
% %\todo{n-1?} 
% according to Eg. \ref{eq:breese}, and supervised learning techniques are suggested for learning $\vec{r}(u,t,n)$ from the aspect ratings $\{\vec{r}(u,t,j): j = 1, ..., n-1\}.$
% %\todo{this is confusing}
% % Both AK and Breese et al. replaced $r(w,t)$ with $r(w,t)-\overline{r_w}$, where $\overline{r_w}$ is the mean of user $w$'s ratings, in Eq. \ref{eq:breese}. 
% % By predicting the variation from the mean, one allows for users whose mean ratings trends high/low.
% % \begin{itemize}
% % \item (Ratings distance)  $d_R(r(u,t), r(v,s)) := \|r(u,t) - r(v,s)\|_p$ for $p =  1, 2, \infty$ (Euclidean, Manhattan, Chebyshev), or Mahalanobis Distance, i.e., $(r(u,t)-r(v,t))^t C (r(u,t) - r(v,t)) $ with $C$ denoting the covariance of $r(\cdot, t) $. 
% % \item (User distance) $d_U(u,v): = \sum_{t\in I_{u,v}} d_R(r(u,t), r(v,t)) /|I_{u,v}|$, with $I_{u,v}:= \{$tools $t$ rated by both $u$ and $v$\}. 
% % \item (User similarity) $\s(u,v) := 1/(1+d_{U}(u,v))$ 
% % \end{itemize}
% %  two methods above are referred to as , as opposed to a progression of 
%  The progression of the research literature diverged from these ``instance-based'' methods to develop ``model-based'' methods, e.g., 
%  \cite{hofmann1999latent, si2003flexible, sahoo2012research}, which  seek Bayesian network models that include latent variables designed to encode clusters of similar users and of items.
% Results of Sahoo et al. \cite{sahoo2012research} conclude that model-based methods excel (in precision-recall balance and in precision-rank balance) when $\vec{r}$ is sparse (common, e.g., in online marketplaces with a huge inventory of items), whereas,  the instance-based method of AK excels
% %(specifically with $\ell^\infty$ ratings distance)\footnote{Through our testing we can provide intuition for why the $\ell^\infty$ ratings norm excels---in this situation, two users are similar  ($\s(u,v)$ small) iff \textit{all} co-rated items are rated similarly. 
% % Thus, predictions are almost exclusively based on those of other users with nearly identical preferences.} 
% for dense $\vec{r}$, which is the case in this study. 



==> 98-acks.tex <==
\section*{Acknowledgements}
Special thanks to Jeff Meredith for assisting with the website. 
The research is based upon work supported by the Department of Defense (DOD), Naval Information Warfare Systems Command (NAVWAR), via the Department of Energy (DOE) under contract  DE-AC05-00OR22725. The views and conclusions contained herein are those of the authors and should not be interpreted as representing the official policies or endorsements, either expressed or implied, of the DOD, NAVWAR, or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes notwithstanding any copyright annotation thereon. 

